Measuring Scale-dependent Shape Anisotropy by Coarse-Graining: Application to Inhomogeneous Rayleigh-Taylor Turbulence

We generalize the `filtering spectrum' [1] to probe scales along different directions by spatial coarse-graining. This multi-dimensional filtering spectrum quantifies the spectral content of flows that are not necessarily homogeneous. From multi-dimensional spectral information, we propose a simple metric for shape anisotropy at various scales. The method is applied to simulations of 2D and 3D Rayleigh-Taylor (RT) turbulence, which is inhomogeneous and anisotropic. We show that 3D RT has clear shape anisotropy at large scales with approximately $4:3$ vertical to horizontal aspect ratio, but tends toward isotropy at small scales as expected [2,3,4]. In sharp contrast, we find that RT in 2D simulations, which are still the main modeling framework for many applications, is isotropic at large scales and its shape anisotropy increases at smaller scales where structures tend to be horizontally elongated. While this may be surprising, it is consistent with recent results in [5]; large-scale isotropy in 2D RT is due to the generation of a large-scale overturning circulation via an upscale cascade, while small scale anisotropy is due to the stable stratification resultant from such overturning and the inefficient mixing in 2D.

==> ref_notes <==
Spectral moments for the analysis of frequency shift, broadening, and wavevector anisotropy in a turbulent fow:
    computing spectra moments in wavenumber-frequency domain and wavevector domain
    elliptic wavevector spectrum 
    non-elliptic wavevector anisotropy model
    shape parameter

The anisotropy present in boundary conditions and large scale forcing is removed in the process of energy cascade to small scales at sufficiently large Reynolds number.

Anisotropy occurs in:
	duct flow (https://doi.org/10.1017/S0022112091000526, Some characteristics of small-scale turbulence in a turbulent duct flow)
	shear flow (The residual anisotropy at small scales in high shear turbulence)
	MHD and plasma (THE ANISOTROPY OF MAGNETOHYDRODYNAMIC TURBULENCE ALFVENIC turbulence)
	solar wind and interstellar turbulence (Anisotropic modal energy transfer in interstellar turbulence)
	passive scalar with large anisotropic forcing (‘Scalar turbulence')
	rotating stratified turbulence (Linking dissipation, anisotropy, and intermittency in rotating stratified turbulence at the threshold of linear shear instabilities)
	4He superfluid (Superfluid Helium in Three-Dimensional Counterflow Differs Strongly from Classical Flows: Anisotropy on Small Scales)
	boundary, forcing, viscosity (Large01JPO)

Anisotropy includes:
	large scale
	inertial range
	small scale: velocity gradients or energy dissipation tensor

Measured by:
	velocity gradients: isotropy imposes some relations among the mean square gradients of different turbulent velocity component as well as the density field, and the deviation from these relations is measured using DNS data of stably stratified turbulent flow. (Assessment of small-scale anisotropy in stably stratified turbulent flows using direct numerical simulations)
	bulk KE in different directions
	structure functions
	energy spectrum tensor
	anisotropic tensor formed by the deviatoric part of the Reynolds stress tensor (2nd and 3rd invariants: https://doi.org/10.1017/S0022112077000585)
	energy spectra in different directions (k_\perp and k_\parallel) (Anisotropy and nonuniversality in scaling laws of the large-scale energy spectrum in rotating turbulence): The authors characterize the anisotropy in rotating turbulence by first decomposing the flow into 2D and 3D (slow and fast) modes, and compared anisotropic spectra of different components associated with each mode.
	deviatoric part of velocity / velocity derivative / scalar / scalar gradient correlation tensor, represented by its tensor invariant quantity
	anisotropic angle (Scaling of anisotropy in hydromagnetic turbulence; Anisotropy in MHD turbulence due to a mean magnetic field): $\theta_Q \equiv \tan^{-1}\{[\Sigma_\bk k_\perp^2 |Q(\bk, t)|^2/\Sigma_\bk k_\parallel^2 |Q(\bk, t)|^2]^{1/2}\}$ where $Q$ is any field variable in Fourier space, and isotropic case corresponds to $\theta=\tan^{-1}(\sqrt{2})$.
	i) co-spectrum of stream-wise velocity u and perpendicular velocity v in homogeneous shear flow, where $E_{uv}(k)$ should vanish for an isotropic flow. and ii) he skewness of the velocity derivative taken in the direction of shear, which should also vanish for isotropic fields. $S_3=\langle (\partial u/\partial y)^3\rangle/\langle (\partial u/\partial y)^2\rangle^{3/2}$. iii) mixed structure function with some particular component occuring odd number of times(Stirring anisotropic turbulence with an active grid)
	By expressing structure functions using spherical harmonics, and deriving the universal scaling exponents for every sector in the irreducible representation of the SO(3) group. In the Kraichnan model of passive scalar advection, this approach yields exact solutions of the scaling exponents, as has also been verified by numerical simulations.
	In reconciling the k^{-5/3} spectrum with small-scale anisotropy observed in many experimental and numerical data, the author adopted the shear-layer model. In the model, any turbulent field is locally recast into the eigenframe of strain-rate tensor at each point, and the velocity fields in the strain eigenframe around all points are averaged to give rise to a so-called "shear layer" structure. Around the center of the shear layer, the solid angle is divided into several bins by splitting the azimuthal angle $\theta$ and elevation angle $\phi$ into different ranges, and then the energy content is averaged inside each bin to give rise to an energy spectrum in the corresponding direction. (The anisotropic structure of turbulence and its energy spectrum)
		

Studying anisotropy because:
	Test the fundamental assumption proposed by Kolmogorov
	Understand the physics of anisotropic flows

Anisotropy in variable density flows

The residual anisotropy at small scales in high shear turbulence: Studied the small-scale anisotropy in wall-bounded flows by decomposing the longitudinal structure function in spherical harmonics, which can seperate different anisotropic contributions. Under strong shear the anisotropy persists to viscous scales. 


Scale-to-scale anisotropy in homogeneous turbulence: The authors studied experimentally the scale-to-scale anisotropy in counterflow jets generated homogeneous turbulence, from the integral scale to the dissipative scales. The integral scale anisotropy is characterized by the axial-to-radial ratio of the root mean square velocity
fluctuations, and also by different integral length scales associated with different velocity components; over the inertial range, the scaling exponents of velocity structure functions differs not only between different components but also between different directions of seperation. At the dissipative scale anisotropy is measured by moments of velocity gradients. They found that the large scale anisotropy persists to dissipative scales.

Compressible Rayleigh–Taylor turbulent mixing layer between Newtonian miscible fluids (velocity spectral anisotropy)

Time-dependent study of anisotropy in Rayleigh-Taylor instability induced turbulent flows with a variety of density ratios:  






points:

1. Isosurface propagating speed, growth rate, reason, single-mode reacceleration

	

瑞利-泰勒不稳定性的混合：ICF， UCC燃烧器，清洁能源，天体物理超新星爆炸，都是可压缩，或者有化学反应

单颗粒两时间拉格朗日速度关联和结构函数,颗粒对分离距离均方和速度关联函数

涡结构的生成、演化和拓扑变化过程,拉格朗日结构函数（二阶，沿水平向或竖向）
相对弥散，湍流混合，促进化学反应

拉格朗日方法研究RT湍流的非各向同性，速度、加速度
加速度自相关函数取不同时间起点的差异

对拟涡能的贡献，时间累计效应，时间相干性

entrainment夹卷,baroclinicity斜压,pressure-dilatation压力--膨胀项,膨胀--耗散项

火焰面粒子追踪，热释放对enstrophy的影响

instantaneous and cumulative (and also combined) effects along Lagrangian trajectories (enstrophy, energy)，涡度拟能（拟涡能）

重力如何影响单个粒子和粒子对的弥散
火焰粒子追踪理论基础
超紧凑燃烧室
自传播曲面

且通过对粒子携带的信息作时间序列关联分析可能有助于找出主导RT各阶段转换的重要物理因素
此外可压缩性[18]和汇聚几何效应[19]对单模RT的影响也逐渐被重视。Hazak[fn3]首次将拉格朗日描述用于分析单模RT，并理论计算了气泡速度的发展。
，h(t)=αAgt^2，其中Atwood数A=(ρ_h-ρ_l)/(ρ_h+ρ_l) 是反映重流体ρ_h和轻流体ρ_l密度比的无量纲数，g为重力加速度，无量纲系数α的取值与初始扰动的波数分布相关，一般只包括高频波数的初始扰动的三维RT中α取值为0.025-0.03，而对于包含低频波数的扰动由于RT对初始条件的记忆性其α取值可达0.06-0.1[20, 21]。 湍流RT的混合层时间

上述Boussinesq描述只适用于轻重流体密度接近的情况，而针对流体密度差别较大的情况或可压缩情况的能量尺度传输也有相关研究[28, 29, 30]，且二维反向能量级串和三维正向能量级串均得以证实。

上述研究中化学反应的时间尺度远小于RT的时间尺度，而Chertkov等人[31]还基于简化的KPP单步反应模型来研究了化学反应速率慢于RT的缓慢反应过程，即Damköhler数小于1的情况。直接数值模拟结果表明，当系统演化时间小于化学反应时间尺度时，可观察到RT的湍流混合作用占主导，而当演化时间更长时，由于化学反应的作用，系统更倾向于呈现单一相的非混合状态，且RT混合层的中心朝燃料区偏移。此外，由于在高离心力超紧凑燃烧器中的应用，非预混的RT燃烧问题也得到相应的关注。Attal和Ramaprabhu[32]研究了单模RT下氢气-空气的非预混燃烧，结果表明火焰面的反应及释热在轻重流体之间增加了第三层流体，结果可能加剧或减缓初始RT问题的稳定性。

鉴于上述研究中火焰锋面在RT问题中的重要性，精细地研究火焰面的几何及拓扑变形规律会对含燃烧RT的深入理解有帮助，因此将拉格朗日粒子法，特别是等值面粒子追踪法应用于本问题有重要意义。

上述工作都表明拉格朗日粒子方法对各类湍流问题研究的独特的贡献，用此方法来研究RT湍流中的涡量场时间历程、粒子加速度统计、粒子弥散等将会是RT问题的一个全新的切入点。 

拟解决：
RT湍流夹卷效应的量化，涡量场对于RT中拟序结构的时间累积效应难以定量刻画，以及RT湍流的物质曲面变化规律难以精确捕捉
中示踪粒子的相对弥散有助于建立RT的湍流混合模型，RT湍流局部火焰推移速度和整体燃烧速度之间的动力学关联，RT不稳定性中的饱和气泡结构再加速，混合层增长率，标度律和间歇性，湍流输运系数建模，以及燃烧RT中火焰锋面变形规律和奇异结构的生成演化等问题

拉格朗日方法独特的优势：量化弥散和混合，entrainment


单模RT粒子clustering，number density, trapping inside vortical structure, correlation of acceleration (centripetal and longtudinal) and vorticity (enstrophy) <=> acceleration autocorrelation, high acceleration associated with strong vortical, trajectory curvature and vorticity, velocity increment along trajectory, jPDF of quantities on trajectories,
vorticity and strain ratio
Lagrangian time-correlation
单模RT：初始粒子的number density随时间变化的contour，背景为isoline
蘑菇区域的strain和vorticity
等值面粒子的切向应变率随时间的变化
potential energy transfer rate and efficiency
单模中交界面竖向和水平向投影面积的比值

从RT达到湍流状态出发，在不同高度seed粒子对，并观察不同高度的涡扩散率与高度的关系
能量释放与界面面积的关系
混合效率与涡量的关系 \rho Y_1 Y_2 / <\rho>
RT湍流中交界面粒子的运动速度与拟涡动能和应变张量的关系
交界面拉伸效应与涡量和应变率的关系
（气泡和尖钉）界面法向量与最大应变率方向的夹角
交界面的厚度
涡量在RT界面如何生成演化的，engulfment, nibbling
获得涡量的流体体积随时间变化
单模RT气泡隔离出来，计算边界线上的压力和剪切应力，计算其受到的总力，看哪一部分贡献最大
单模RT的mixing
加速度和轨迹curvature之间的关系
nabla rho nabla P夹角分布
水平方向能量的转换
条件统计 Y1 Y2>0.1
S_ij的特征向量方向与grad rho, grad P夹角
S_ij特征值大小
Q-R相图
涡量与夹角的joint PDF
粒子轨迹曲率与涡量的jPDF

Mantzaras and Frouzakis ProCI 2019 adopted the platinum surface reaction mechanism by Deutschmann2000, which is characterized by fast depletion of reactants, while the mechanism adopted in our work is adapted from Aghalayam et al CTM 1998, characterized by rapid radical adsorption (see Saiki and Suzuki ProCI 2013 for more details).  Our research direction would focus on the local extinction of near-wall turbulent flames due to radical quenching, thus we chose the Aghalayam mechanism to provide us with the upper limit of radical depletion effects. In addition, our aim is to study the behavior of general reactive surfaces instead of platinum-coated walls (although the site density is chosen to be close to platinum), this kind of `idealized' surface mechanism has been chosen by many previous works (mostly on H2/air and CH4/air flames, see Raimondeau et al. ProCI 2002, Hua et al. Chemical Engineering Science 2005, Kizaki et al. ProCI 2015, Narukawa et al. Fuel 2020). We would also adopt the Deutschmann mechanism in our future work to compare the Pt-coated wall with our current results. We will revise our draft to include additional motivations for us to use the current surface mechanism.

Due to the high radical adsorption and surface recombination rates in our adopted mechanism, the near wall H radicals would be transformed to H2 by the reactive wall, thus in the reactive wall case the near-wall H2 mass fraction is slightly larger than the inert wall case, which should be quite different from the Deutschmann Pt mechanism, as is pointed out by the reviewer. For the wall temperature, as we have argued in the draft, the heat from recombination of adsorbed radicals releases extra energy back to the gas phase through the additional wall heat flux, which offsets the low gas-phase HRR near the reactive wall. But we do observe increases in wall temperature differences as the ambient temperature is increased (1% relative wall-temperature difference at 300K ambient temperature, while 4% relative difference is observed for 1200K ambient temperature).

Compared to other DNS simulations involving surface reactions, such as Mantzaras and Frouzakis ProCI 2019, the most distinctive difference is that our configuration is a head-on quenching one, while others mainly focus on side-wall quenching. The effects of surface reactions on the flame would be different for the two cases. We will implement the more realistic Pt catalytic mechanism to check the differences with our current results. Also, we thank the reviewer for providing us additional up-to-date references, which we shall include in our revised draft.



Our study is to investigate general reactive surface instead of platinum-coated walls (although the site density is chosen to be close to platinum),  and our further research direction would focus on near-wall turbulent local flame extinction due to radical quenching.

The major difference 


1. Our study is to investigate general reactive surface instead of platinum-coated walls (although the site density is chosen to be close to platinum),  and our further research direction would focus on near-wall turbulent local flame extinction due to radical quenching. The particular reaction mechanism we have chosen (Aghalayam et al, Combust. Theor. Model. 1998) provides a rapid adsorption of radicals, thus setting an upper bound for radical quenching to occur in the gas phase. 

does not include the dissociative adsorption of H2 and O2



利用Richardson数，区分RTI region和KHI region，进行速度统计
